Self-Healing Hybrid Control as a Proxy for Detection and Mitigation of Sensor Attacks in Cooperative Driving

We propose a real-time hybrid controller scheme to detect and mitigate False-Data Injection (FDI) attacks on Cooperative Adaptive Cruise Control (CACC). Our method uses sensor redundancy to create equivalent controller realizations, each driven by distinct sensor subsets but producing identical control inputs when no attack occurs. By comparing control signals and measurements via majority voting, the scheme identifies compromised sensors in real-time and switches to a healthy controller, even under unconstrained attacker switching. The hybrid controller utilizes attack-dependent flow and jump sets, and resets the states of compromised controllers, resulting in a self-healing architecture. Simulation results demonstrate the effectiveness of this approach.

==> 0.Bibligraphy.tex <==
\bibitem{ploeg_design_2011}
J. Ploeg, B. T. M. Scheepers, van Nunen, N. van de Wouw, and H. Nijmeijer, "Design and Experimental Evaluation of Cooperative Adaptive Cruise Control", in \textit{IEEE Conference on Intelligent Transportation Systems (ITSC)}, p. 260--265, 2011.

\bibitem{el-rewini_cybersecurity_2020}
Z. El-Rewini, K. Sadatsharan, D. F. Selvaraj, S. J. Plathottam, and P. Ranganathan, "Cybersecurity Challenges in Vehicular Communications", in \textit{Vehicular Communications}, vol. 23, p. 100214, 2020.

\bibitem{ju_survey_2022}
Z. Ju, H. Zhang, X. Li, X. Chen, J. Han, and M. Yang, "A Survey on Attack Detection and Resilience for Connected and Automated Vehicles: From Vehicle Dynamics and Control Perspective," in \textit{IEEE Transactions on Intelligent Vehicles}, vol. 7, p. 815--837, 2022.

\bibitem{sun_survey_2022}
X. Sun, F. R. Yu, and Z. Zhang, "A Survey on Cyber-Security of Connected and Autonomous Vehicles (CAVs)", in \textit{IEEE Transactions on Intelligent Transportation Systems}, vol. 23, no. 7, p. 6240--6259, 2022.

\bibitem{chowdhury_attacks_2020}
A. Chowdhury, G. Karmakar, J. Kamruzzaman, A. Jolfaei, and R. Das, "Attacks on Self-Driving Cars and Their Countermeasures: A Survey", in \textit{IEEE Access}, vol. 8, p. 207308--207342, 2020.

\bibitem{chong_observability_2015}
M. S. Chong, M. Wakaiki, and J. P. Hespanha, "Observability of linear systems under adversarial attacks", in \textit{Proc. Amer. Control Conf. (ACC)}, pp. 2439-2444, 2015.

\bibitem{fawzi_secure_2014}
H. Fawzi, P. Tabuada, and S. Diggavi, "Secure Estimation and Control for Cyber-Physical Systems Under Adversarial Attacks", in \textit{IEEE Transactions on Automatic Control}, vol. 59, pp. 1451--1467, 2014. 

\bibitem{ding_secure_2021}
D. Ding, Q. Han, X. Ge, and J. Wang, "Secure State Estimation and Control of Cyber-Physical Systems: A Survey", in \textit{IEEE Transactions on Systems, Man, and Cybernetics: Systems}, vol. 51, pp. 176 -- 190, 2021.

\bibitem{niazi_resilient_2023}
M. U. B. Niazi, A. Alanwar, M. S. Chong, and K. H. Johansson, "Resilient set-based state estimation for linear time-invariant systems using zonotopes", in \textit{European Journal of Control}, vol. 74, pp. 100837, 2023.

\bibitem{petri_towards_2022}
E. Petri, R. Postoyan, D. Astolfi, D. Nesic, and V. Andrieu, "Towards improving the estimation performance of a given nonlinear observer", in \textit{61st Conference on Decision and Control}, pp. 583--590, 2022.

\bibitem{lu_secure_2017}
A. Lu, and G. Yang, "Secure state estimation for cyber-physical systems under sparse sensor attacks via a switched Luenberger observer", in \textit{Information Sciences}, v. 417, pp. 454--464, 2017. 

\bibitem{van_der_heijden_analyzing_2017}
R. van der Heijden, T. Lukaseder, and F. Kargl, "Analyzing Attacks on Cooperative Adaptive Cruise Control (CACC)", in \textit{IEEE Vehicular Networking Conference (VNC)}, p. 45--52, 2017.

\bibitem{mao_computational_2022}
M. Yanwen, A. Mitra, S. Sundaram, and P. Tabuada, "On the computational complexity of the secure state-reconstruction problem", in \textit{Automatica}, vol. 136, p. 110083, 2022.

\bibitem{huisman_optimal_2024}
M. Huisman, C. Murguia, E. Lefeber, and N. van de Wouw, "Optimal Controller Realizations Against False Data Injections in Cooperative Driving", in \textit{63nd IEEE Conference on Decision and Control (CDC)}, 2024.

\bibitem{sanfelice_toolbox_2013}
R. G. Sanfelice, D. A. Copp, and P. Nanez, "A toolbox for simulation of hybrid systems in Matlab/Simulink: hybrid equations (HyEQ) toolbox," in \textit{Proc. of the 16th international conf. on Hybrid systems: computation and control}, pp. 101--106, 2013.

\bibitem{goebel_hybrid_2012}
R. Goebel, R.G. Sanfelice, and A.R. Teel, "Hybrid dynamical systems: modeling, stability, and robustness", Princeton University Press, 2012.

\bibitem{anand_risk_2022}
S. C. Anand, A. M. H. Teixeira, and A. Ahlen, "Risk assessment and optimal allocation of security measures under stealthy false data injection attacks", in \textit{2022 IEEE Conference on Control Technology and Applications (CCTA)}, p. 1347–-1353, 2022.












\begin{comment}
\bibitem{ploeg_graceful_2013}
J. Ploeg, E. Semsar-Kazerooni, G. Lijster, N. van de Wouw, and H. Nijmeijer, "Graceful Degradation of {CACC} Performance Subject to Unreliable Wireless Communication", in \textit{IEEE Conference on Intelligent Transportation Systems (ITSC)}, p. 1210--1216, 2013.

\bibitem{lefeber_cooperative_2020}
E. Lefeber, J. Ploeg, and H. Nijmeijer, "Cooperative Adaptive Cruise Control of Heterogeneous Vehicle Platoons", in \textit{IFAC-PapersOnLine}, vol. 53, no. 2, p. 15217--15222, 2020. 

\bibitem{amoozadeh_security_2015}
M. Amoozadeh, A. Raghuramu, C. Chuah, D. Ghosal, M. Zhang, J. Rowe, and K. Levitt, "Security Vulnerabilities of Connected Vehicle Streams and Their Impact on Cooperative Driving", in \textit{IEEE Communications Magazine}, vol. 53, p. 126--132, 2015.

\bibitem{teixeira_secure_2015}
A. Teixeira, I. Shames, H. Sandberg, and K. H. Johansson, "A Secure Control Framework for Resource-Limited Adversaries, in \textit{Automatica}, vol. 51, p. 135--148, 2015.

\bibitem{teixeira_attack_2012}
A. Teixeira, D. Pérez, H. Sandberg, and K. H. Johansson, "Attack models and scenarios for networked control systems", in \textit{Proceedings of the 1st international conference on High Confidence Networked Systems}, p. 55-64, 2012.

\bibitem{zhang_networked_2019}
X.-M. Zhang, Q.-L Han, X. Ge et al., "Networked Control Systems: A Survey of Trends and Techniques", in \textit{IEEE/CAA Journal of Automotica Sinica}, p. 1-17, 2019. 

\bibitem{teixeira_strategic_2015}
A. Teixeira, H. Sandberg and K. H. Johansson, "Strategic stealthy attacks: The output-to-output L2-gain", in \textit{2015 54th IEEE Conference on Decision and Control (CDC)}, p. 2582–-2587, 2015. 

\bibitem{wolf_securing_2020}
M. Wolf, A. Willecke, J.-C. Muller et al., "Securing CACC: Strategies for Mitigating Data Injection Attacks", in \textit{2020 IEEE Vehicular Networking Conference (VNC)}, p. 1–7, 2020.

\end{comment}

==> 2_Preliminaries/2.1_Notation.tex <==
\subsection{Notation} \vspace{-1.5mm}
The symbol $\mathbb{R}$ stands for the real numbers, $\mathbb{R}_{>0}$ ($\mathbb{R}_{\geq 0}$) denotes the set of positive (non-negative) real numbers. The symbol $\mathbb{N}$ denotes the set of natural numbers, including zero. The $n \! \times \! m$ matrix composed of only zeros is denoted by $\mathbf{0}_{n \times m}$, or $\mathbf{0}$ when its dimension is clear. Time dependencies of signals are often omitted for simplicity of notation.
 


==> 2_Preliminaries/2.2_Definition.tex <==
\subsection{Definitions} \vspace{-1.5mm}
%%% DEFENITION 1 (REACHABLE SET) %%%
\begin{definition}[Hybrid Dynamical System]\emph{\cite{goebel_hybrid_2012}}\label{DefHybridSystem}
Consider the hybrid dynamical system:
\begin{align} \label{eq:HybridGeneral}
    \left\{ \begin{aligned}
    \dot{x} &= f(x,u), \text{ if }(x,u)\in \mathcal C, \\
        x^+ &= g(x,u), \text{ if }(x,u)\in \mathcal D,
    \end{aligned} \right.
\end{align}
where $x\in \mathbb R^{n_x \times 1}$ is the state vector, $\dot x$ represents its continuous evolution, and $x^+$ denotes the state after an instantaneous jump. The input vector is given by $u \in \mathbb R^{n_u}$. The function $f(x,u)$ defines the flow map and $g(x,u)$ represents the jump map, with their corresponding flow set $\mathcal C$, and jump set $\mathcal D$, respectively. The solutions of \eqref{eq:HybridGeneral} evolve over a hybrid time domain $(t,j) \in \mathbb E$ where $t$ represents continuous time, and $j$ represents the discrete jump counter. The subset $\mathbb E \subset \mathbb R_{>0} \times \mathbb N$ is called a \textit{compact hybrid time domain} if $\mathbb E = \bigcup^J_{j=0}([t_j, t_{j+1}],j)$ for some finite sequence of times $0 = t_0 \leq ... \leq t_{J+1}$. We say $\mathbb E$ is a \textit{hybrid time domain} if, for each $(T,J)\in \mathbb E$, the intersection $\mathbb E \bigcap([0,T] \times \{0,...,J\})$ is a compact hybrid time domain.
\end{definition}
%%% END DEFENITION 1 (Hybrid Dynamical System) %%%





==> 3_ProblemSetting/3.1_ProblemSetting.tex <==
Consider a homogeneous platoon of $m$ vehicles, as illustrated in Fig.~\ref{fig:Platoon}. The vehicles are indexed by $i=1,...,m,$ where $i=1$ indicates the lead vehicle. To describe the platooning behavior, we adopt a linear platooning model \cite{ploeg_design_2011}:
\begin{align} \label{eq:SD_PlatoonDynamics}
    \begin{bmatrix}
        \dot{v}\imo \\ \dot{a}\imo \\ \dot{d}_i \\ \dot{v}_i \\\dot{a}_i
    \end{bmatrix}
    = 
    \begin{bmatrix}
        a\imo \\ -\tfrac{1}{\tau}\aim + \tfrac{1}{\tau} \uim \\ \vim - v_i \\ a_i \\ -\frac{1}{\tau}a_i + \frac{1}{\tau} u_i
    \end{bmatrix}, \, i \in S_m \backslash \{1\},
\end{align}
where $d_i = q_{i-1} - q_i - L_i$ is the distance between vehicle $i$ and its preceding vehicle $i-1$, with $q_i$ denoting the position of the vehicle's rear bumper, and $L_i$ its length. Furthermore, $v_i$ and $a_i$ denote the velocity and acceleration of vehicle $i$, respectively, and $S_m \coloneqq \{ i \in \mathbb{N} \mid 1 \leq i \leq m \}$ (i.e., the set of all vehicles in a platoon of length $m \in \mathbb{N}$). The desired acceleration $u_i$ represents the control input of vehicle $i$, and $\tau>0$ is a time constant modeling driveline dynamics.

Each vehicle in $S_m$ is equipped with onboard sensors (e.g., LiDAR, cameras, and velocity/acceleration sensors) and wireless V2V communication to receive data from adjacent vehicles. Considering a combination of sensors, we assume to have access to the following sensor data:
\begin{align} \vspace{-4mm}  \label{eq:SD_Sensors}
    \begin{aligned}
        y_{i,1} &\coloneqq d_i + \delta_{i,1}, 
        \ \ \ \ \ \ \ \ y_{i,2} \coloneqq v_i + \delta_{i,2}, \\
        y_{i,3} &\coloneqq a_i + \delta_{i,3}, 
        \ \ \ \ \ \ \ \ y_{i,4} \coloneqq v_{i-1} - v_i + \delta_{i,4}, \\
        y_{i,5} &\coloneqq a_{i-1} + \delta_{i,5}, 
        \ \ \ \ \ y_{i,6} \coloneqq u_{i-1} + \delta_{i,6}.
    \end{aligned}
\end{align} \vspace{0mm} 
Herein, $\delta_{i,j}$ models potential FDI attacks. Furthermore, sensors $y_{i,1}$ and $y_{i,4}$ provide relative distance and velocity information, $y_{i,2}$ and $y_{i,3}$ are the onboard measured velocity and acceleration, while $y_{i,5}$ and $y_{i,6}$ represent the wirelessly received data from the preceding vehicle. 
\begin{figure}[bt]\centering
		\includegraphics[width=\linewidth]{00_Figures/PlatoonReduced.eps} \vspace{-1mm}
		\caption{Vehicle platoon with CACC. Each vehicle has onboard sensors (e.g., LiDARs, cameras, and velocity/acceleration sensors) which may be subject to FDI attacks.}
		\centering
		\label{fig:Platoon}
  \vspace{0mm}
\end{figure}

The control objective for each follower vehicle is to keep a desired inter-vehicle distance $d_{r,i} = r + h v_i, \, i \in S_m \backslash \{ 1 \}$, with time gap $h>0$, and standstill distance $r>0$. The spacing error is defined as $e_i \coloneqq d_i - d_{r,i}$. To ensure this desired spacing and achieve string-stable vehicle-following behavior, a CACC scheme is introduced for a homogeneous platoon in \cite{ploeg_design_2011}. The proposed CACC scheme is a dynamic controller of the following form:
\begin{align} 
\label{eq:SD_BaseController} \vspace{-2mm} 
        \mathcal{F} &\coloneqq \left\{ 
            \begin{aligned}
                u_i &= \rho_i, \\
                \dot{\rho}_i &= -\tfrac{1}{h} \rho_i + \tfrac{1}{h}(k_p e_i + k_d \dot{e}_i) + \tfrac{1}{h} \uim,
            \end{aligned} \right.           
\end{align}
where $k_p>0$ and $k_d>0$ are control gains to be designed.

To enhance the robustness of the CACC scheme in~\eqref{eq:SD_BaseController} against the FDI attacks in~\eqref{eq:SD_Sensors}, we propose a hybrid control framework that exploits equivalent controller realizations, i.e., different realizations producing the same control input~$u$ while using different sensors. These realizations depend on distinct minimal sensor sets, enabling redundancy for attack detection and mitigation without constraining the attacker's switching frequency. 

Our contributions are: 1) a method to construct two distinct minimal-sensor equivalent controller realizations, and 2) an attack detection and mitigation scheme that switches between these realizations, ensuring a healthy control input is always applied. Additional stability analysis is not required, since the base controller~\eqref{eq:SD_BaseController} already guarantees the desired closed-loop performance.
\vspace{-1mm}



==> 4_Approach/4.1_ControllerRealizationsV2.tex <==
This section derives controller realizations that enable a hybrid control scheme for detecting FDI attacks. Using the sensor measurements $y_i=[y_{i,1}, \dots, y_{i,6}]^\top$, we define a new controller state $\bar{\rho}_i$ via the proposed linear change of coordinates in \cite{huisman_optimal_2024}: 
\begin{align} \label{eq:CR_Transformation}
  \bar{\rho}_i &=  \rho_i + \underbrace{\begin{bmatrix} \beta_{i,1} & \beta_{i,2} & \beta_{i,3} & \beta_{i,4} & \beta_{i,5} & 0 \end{bmatrix}}_{\beta_i} y_i.
\end{align}
This transformation yields a class of equivalent controller realizations, i.e., controllers that produce the same control input $u_i$ while using different sensors. Applying~\eqref{eq:CR_Transformation} to the CACC controller~\eqref{eq:SD_BaseController} yields the equivalent CACC controllers:
\begin{subequations}\label{eq:rhoBar} \vspace{0mm}  \begin{align} 
    u_i &= \bar\rho_i - \beta_i y_i, \\
    \dot{\bar{\rho}}_i &= -\left(\tfrac{1}{h} + \tfrac{\beta_{i,3}}{\tau} \right)
 \bar\rho_i + \sum\nolimits_{j=1}^{6} \bar B_{i,j} y_{i,j}, \\
     \bar B_{i,1} &= -\tfrac{\beta_{i,1} \beta_{i,3}}{\tau}-\tfrac{\beta_{i,1}}{h}+\tfrac{k_p}{h},\\
     \bar B_{i,2} &= -\tfrac{\beta_{i,2} \beta_{i,3}}{\tau}-\tfrac{\beta_{i,2}}{h}-k_p,\\
     \bar B_{i,3} &= \beta_{i,4}-\tfrac{\beta_{i,3}^2}{\tau}-\beta_{i,2}+\tfrac{\beta_{i,3}}{\tau}-\tfrac{\beta_{i,3}}{h}-k_d,\\
     \bar B_{i,4} &= \tfrac{k_d}{h}-\tfrac{\beta_{i,4} \beta_{i,3}}{\tau}-\beta_{i,1}-\tfrac{\beta_{i,4}}{h},\\
     \bar B_{i,5} &= \tfrac{\beta_{i,5}}{\tau}-\tfrac{\beta_{i,5} \beta_{i,3}}{\tau}-\beta_{i,4}-\tfrac{\beta_{i,5}}{h},\\
     \bar B_{i,6} &= \tfrac{1}{h}-\tfrac{\beta_{i,5}}{\tau}. 
 \end{align} \end{subequations} \vspace{-5mm} 

Although $y_i$ comprises six sensor measurements, we first seek to minimize the sensor dependency. Reducing the number of sensors lowers both redundancy and security requirements~(\cite{anand_risk_2022}). This is achieved by finding pairs ($\beta_{i,j},\bar{B}_{i,j}$) equal to zero, where $\beta_{i,j} = 0$ ensures that the sensor is not required in \eqref{eq:CR_Transformation}, and $\bar{B}_{i,j}$ excludes the sensor in \eqref{eq:rhoBar}. For example, excluding $y_{i,1}$ requires
\begin{align} \vspace{-1mm}
    \beta_{i,1} &= 0, \quad 
    \bar{B}_{i,1} = -\tfrac{\beta_{i,1} \beta_{i,3}}{\tau}-\tfrac{\beta_{i,1}}{h}+\tfrac{k_p}{h} = 0,
\end{align}
which has no solution for $h,k_p>0$, indicating that $y_{i,1}$ is always required to realize the controller. In contrast, excluding $y_{i,6}$ is possible by satisfying
\begin{align}  \label{eq:beta5_y5} \vspace{-1mm}
    \bar B_{i,6} &= \tfrac{1}{h}-\tfrac{\beta_{i,5}}{\tau} =0,
\end{align} 
implying $\beta_{i,5} = \tfrac{\tau}{h}$. This result also implies that excluding both $y_{i,5}$ and $y_{i,6}$ is impossible as this would require $\beta_{i,5} = 0$. Similar results hold for other sensors, but we omit the detailed derivations for brevity.

Following this approach, we obtain two controller realizations $\mathcal{F}_{i,1}$ and $\mathcal{F}_{i,2}$ by selecting $\beta_{i,1} = [\tfrac{k_d}{h} \, -k_d \, 0 \, 0 \, \tfrac{\tau}{h} \, 0]$ and $\beta_{i,2} = [ \tfrac{k_d}{h} \, {-k_d} \, 0 \, 0 \, 0 \, 0]$, respectively, which yield:
\begin{subequations} \label{eq:Ci1Ci2} \begin{align}
    \mathcal F_{i,1}&= \left\{ 
    \begin{aligned} 
        \dot \rho_{i,1} &=  -\tfrac{1}{h}\rho_{i,1} +\left(\tfrac{k_p}{h} -\tfrac{k_d}{h^2}\right)\,y_{i,1} \\ & -\left(k_p-\tfrac{k_d}{h}\right)y_{i,2} -\left(\tfrac{\tau }{h^2}-\tfrac{1}{h}\right)y_{i,5}, \\
        u_{i,1} &= \rho_{i,1} + \tfrac{k_d}{h} y_{i,1} - k_d y_{i,2}+\tfrac{\tau}{h}y_{i,5},
    \end{aligned}
    \right. \\ %\end{align} \begin{align}
    \mathcal F_{i,2}&= \left\{ 
    \begin{aligned}
        \dot \rho_{i,2} &= -\tfrac{1}{h}\rho_{i,2} + \left(\tfrac{k_p}{h}-\tfrac{k_d}{h^2}\right)y_{i,1} \\
        &- \left(k_p-\tfrac{k_d}{h}\right)y_{i,2} +\tfrac{1}{h}y_{i,6}, \\
        u_{i,2} &= \rho_{i,2} + \tfrac{k_d}{h} y_{i,1} -k_d y_{i,2},
    \end{aligned}
    \right. 
\end{align}\end{subequations}
with the new controller states $\rho_{i,1}$ and $\rho_{i,2}$. As seen in \eqref{eq:Ci1Ci2}, these controller realizations require only three sensors: either $\mathcal{Y}_{i,1} = \{ y_{i,1}, y_{i,2},y_{i,5}\}$, or $\mathcal Y_{i,2} = \{y_{i,1}, y_{i,2},y_{i,6}\}$. Since these realizations are independent of the vehicle index $i$, there is no longer a need to distinguish between vehicles $i$ and $i-1$. Therefore, the subscript $i$ is omitted for clarity.  
\begin{assumption} \label{ass:one_attack}
The attacker may switch between sensors arbitrarily, but may compromise (i.e., $\delta_{i,j}\neq0$) only one sensor at any given time.
\end{assumption}
Under Assumption~\ref{ass:one_attack}, we show how $\mathcal{F}_{i,1}$ and $\mathcal{F}_{i,2}$ can be used to reduce sensor redundancy requirements through majority voting. Let $y_{j|k}$ denote measurement $j$ from physical sensor $k$, and $\mathcal{Y} ~= \{y_{1|1}, y_{1|2}, y_{1|3}, y_{2|1}, y_{2|2}, y_{2|3}, y_{5|1}, y_{5|2}, y_{6|1}, y_{6|2}\}$ defines the sensor set. For instance, $y_{1|1}$ is obtained via LiDAR, while $y_{1|2}$ and $y_{1|3}$ are obtained via different cameras. Through majority voting, the true value of $y_1$ and $y_2$ can be extracted under Assumption~\ref{ass:one_attack}. For instance, if $y_{1|3}$ is compromised, we can recover $y_1$ by relying on the majority, since $y_{1|1} = y_{1|2} \neq y_{1|3}$. A similar reasoning applies to $y_2$. However, for $y_5$ and $y_6$, where only two physical sensors are available, majority voting is inconclusive when $y_{4+j|1} \neq y_{4+j|2}, \,j \in \{1,2\}$. 

Instead of adding a third sensor $y_{4+j|3}$, we exploit the controller realizations in~\eqref{eq:Ci1Ci2}. Assuming the true value of $y_1$ and $y_2$ are obtained via majority voting, we redefine the sensor set $\mathcal{Y} = \{y_1, y_2, y_{5|1}, y_{5|2}, y_{6|1}, y_{6|2}\}$, and obtain four distinct controller realizations for $k \in \{1,2\}$:
\begin{subequations} \label{eq:C1zC2z} \begin{align}
    \mathcal F_{1|k}&= \left\{ 
    \begin{aligned} 
        \dot \rho_{1|k} &=  -\tfrac{1}{h}\rho_{1|k} +\left(\tfrac{k_p}{h} -\tfrac{k_d}{h^2}\right)\,y_{1} \\ & -\left(k_p-\tfrac{k_d}{h}\right)y_{2} -\left(\tfrac{\tau }{h^2}-\tfrac{1}{h}\right) y_{5|k}, \\
        u_{1|k} &= \rho_{1|k} + \tfrac{k_d}{h} y_{i,1} - k_d y_{2}+\tfrac{\tau}{h} y_{5|k},
    \end{aligned}
    \right. \\
    \mathcal F_{2|k}&= \left\{ 
    \begin{aligned}
        \dot \rho_{2|k} &= -\tfrac{1}{h}\rho_{2|k} + \left(\tfrac{k_p}{h}-\tfrac{k_d}{h^2}\right)y_{1} \\
        &- \left(k_p-\tfrac{k_d}{h}\right)y_{2} +\tfrac{1}{h} y_{6|k}, \\
        u_{2|k} &= \rho_{2|k} + \tfrac{k_d}{h} y_{1} -k_d y_{2},
    \end{aligned}
    \right. 
\end{align}\end{subequations}
where $\rho_{1|k}$ and $\rho_{2|k}$ denote the new controller states and $k$ denoting which sensor is used. For example, $\mathcal F_{1|1}$ utilizes $y_{5|1}$, and $\mathcal F_{1|2}$ utilizes $y_{5|2}$. Since these controller realizations are equivalent in the absence of an attack, the following holds
\begin{subequations} \vspace{0mm} \label{eq:RealizationProperties}
    \begin{align} 
        u_{1|1} &= u_{1|2} = u_{2|1} = u_{2|2}, \\
        \implies \rho_{1|1} + \tfrac{\tau}{h} y_{5|1} &= \rho_{1|2} + \tfrac{\tau}{h}y_{5|2} =  \rho_{2|1} = \rho_{2|2}. 
    \end{align}
\end{subequations}
Violations of the equalities in~\eqref{eq:RealizationProperties} indicate an FDI attack, i.e, $\delta_{4+j|k} \neq 0, \, j,k \in \{1,2\}$. The next section presents a hybrid control scheme that leverages the controller realizations~\eqref{eq:C1zC2z} and its properties~\eqref{eq:RealizationProperties} to identify the compromised sensors.

